Machine Learning Fairness for Depression Detection using EEG Data

This paper presents the very first attempt to evaluate machine learning fairness for depression detection using electroencephalogram (EEG) data. We conduct experiments using different deep learning architectures such as Convolutional Neural Networks (CNN), Long Short-Term Memory (LSTM) networks, and Gated Recurrent Unit (GRU) networks across three EEG datasets: Mumtaz, MODMA and Rest. We employ five different bias mitigation strategies at the pre-, in- and post-processing stages and evaluate their effectiveness. Our experimental results show that bias exists in existing EEG datasets and algorithms for depression detection, and different bias mitigation methods address bias at different levels across different fairness measures.

==> content/Angus_thesis.tex <==
%\chapter{Introduction}
%\section{Introduction, Background and Motivation}
\section{Introduction}
%\raggedbottom
\label{chap:intro}

%\label{firstcontentpage} % start page count here


%\section{Background and Motivation}

Mental disorders, such as major depressive disorders (MDD), are affecting more people around the world. MDD, also known as clinical depression, is the most common type of depressive disorder\footnote{Nevertheless, MDD is often used interchangeably with depression, also known as depressive disorder. We follow this convention as well.} \cite{1990_2017} that is characterised by depressed mood, loss of interest or pleasure and other symptoms over at least two weeks \cite{dsm5}. During the first year of the COVID-19 pandemic, the number of people with MDD increased by 28\% to around 246 million \cite{who}. Depression has further implications for individuals and society. It is not only a risk factor for diabetes and coronary heart disease \cite{who_europe}, but also one of the major contributors to global disability and suicide deaths \cite{who_booklet}. Furthermore, it creates a great economic and social burden \cite{burden}. Therefore, it is important to identify depressed individuals for early and effective treatment. However, clinical characterisation of depression is often ineffective due to the absence of objective diagnostic criteria \cite{clinical, ml_eeg}. As an alternative, ML, especially deep learning (DL), has been recently used in many research studies for depression detection with success \cite{ml_eeg, dl_eeg}. In these studies, the use of EEG data is common. Since they are associated with the electrical activity of the human brain, they are considered one of the most valuable tools for depression detection \cite{dl_eeg}.

Meanwhile, there has been more research in the field of ML fairness in the past decade \cite{eq_opp,corbett2017algorithmic}. Informally, fairness means that no individual or group should be advantaged or disadvantaged based on their inherent characteristics, and bias is considered its opposite \cite{bias_survey}. As ML is used more extensively in automated decision-making for job recruitment \cite{kochling2020discriminated}, % university admissions, 
recidivism prediction \cite{corbett2017algorithmic}, etc., there is growing attention towards the fairness of ML algorithms. In fact, one main concern over the use of ML-based depression detection is the potential bias of ML algorithms \cite{concern}. This would violate justice, one of the principles of clinical ethics, which states that all patients should be treated equally and equitably \cite{clinical_ethics}. Consequently, there is little use of ML techniques in the clinical diagnosis of depression. Indeed, only a limited number of studies on ML fairness for mental health (MH) analysis have been carried out \cite{jiaee, mhbias}. Specifically, there has been no investigation on ML fairness using EEG data at the point of writing. Therefore, it is crucial to understand and evaluate the fairness of different ML models in depression detection so that existing bias can be mitigated. This helps alleviate the concern that such methods might discriminate against certain demographic groups and promote the use of related technologies on a larger scale for the benefit of people. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}

\section{Research Questions (RQs)}
\label{sec:RQ}
The above motivates the following RQs of this work: 
\begin{enumerate}[label=\textbf{RQ\arabic*.}, leftmargin=*]
    \item \textbf{Is there bias in existing EEG-based depression datasets and algorithms?} \\
To investigate this issue, we train existing models using different datasets and evaluate their \textbf{gender} fairness (and performance). We focus on \textbf{DL models} in this study. 
    \item \textbf{What is the performance-fairness trade-off of existing bias mitigation strategies?} \\
To answer this question, we carry out various bias mitigation strategies. We then re-evaluate the performance and fairness and contrast the results with those before the strategies are performed. 
    \item \textbf{Can we make existing EEG-based depression detection algorithms fairer while accurate?} \\
The observations from answering RQ2 suggest which strategies are more promising than others. Building on top of these findings, we propose a new bias mitigation strategy with the goal of improving fairness without largely compromising performance. The proposed method is compared with existing methods. 
\end{enumerate}

\end{comment}

\section{Contributions}
%In line with the RQs stated, we make the following contributions:
\begin{itemize}
    \item This study is the first attempt to evaluate ML fairness for depression detection using EEG data, as far as the author is aware. We show that bias exists in published datasets and algorithms. 
    \item None of the existing work on ML fairness for depression detection \cite{jiaee, aguirre, postpartum, Bailey_Plumbley_2021} has investigated bias mitigation for depression detection using EEG data. We study and compare the effectiveness of a diverse set of bias mitigation techniques, which span different stages of the training process, in improving fairness in EEG-based depression detection. We show they have different effects on performance and fairness. 
    \item We propose an improved regularisation-based bias mitigation approach to achieve a better performance-fairness balance. We benchmark our proposed method against other methods for three models across three datasets.
\end{itemize}

\begin{comment}

\section{Dissertation Structure}
The rest of the dissertation is structured as follows. Chapter \ref{chap:background} covers background material or related work on the key terms of this study, including DL, depression detection, EEG, ML fairness and bias mitigation. Chapter \ref{chap:methodology} describes our methodology. In particular, we detail the metrics and bias mitigation methods used, including the proposed method. Chapter \ref{chap:setup} introduces the experimental setup and covers details of the datasets, models and implementation. In Chapter \ref{chap:results}, we present the experimental results followed by a discussion of the results. Finally, we provide a summary, introduce the limitations and conclude the work in Chapter \ref{chap:concl}. 

%\chapter{Background and Related Work}
%\label{chap:background}
\emph{This chapter expands on the key terms of the project. The first part introduces the field of automatic depression detection, starting from a generic outline with a description of relevant DL architectures to a more focused description of EEG data and EEG-based methods. The second part is related to fairness, where various criteria and definitions of fairness and bias mitigation strategies are detailed. It also covers some existing work on fairness in MH-related applications.} 

\section{Automatic Depression Detection (ADD)}
We begin with some background material on DL. This will provide a foundation for the understanding of ADD introduced later.
\end{comment}


\begin{comment}

\subsection{DL Techniques}
DL is a subfield of ML that is based on artificial neural networks with multiple hidden layers. DL models can learn complex non-linear functions and extract high-level features automatically from data, hence reducing the need for feature engineering. This section provides a brief overview of some DL architectures that are particularly useful \cite{dl_time_series, dl_time_series_review} for \emph{time-series} data, which means the input features are ordered chronologically \cite{time_series}. 

\subsubsection{Convolutional Neural Networks (CNNs)}
CNNs are a commonly used architecture which performs particularly well for image-based tasks \cite{khan2018guide, goodfellow2016deep} and they can be used to process arrays with other dimensions. Some common applications include object recognition, image segmentation and medical image analysis \cite{bernal2019deep,schirrmeister2017deep}. CNNs use much fewer parameters than fully connected networks to accomplish the same task.

The key feature of CNNs is \emph{convolutional layers}. They comprise a set of \emph{kernels}, or \emph{filters} which are arrays with learnable weights. The operation of convolutional layers is to calculate the dot product of the kernel weights and the elements of the tensor (e.g.\ pixel values) in a local patch as the kernel is slid across the input tensor (e.g.\ an image). These products form a \emph{feature map}. The sliding distance known as \emph{stride} is specified and some padding is usually applied at the boundaries. Convolutional layers are sometimes followed by \emph{pooling layers}, which perform aggregation such as maximisation or averaging in local patches. The stride is typically larger to achieve downsampling. 

The kernels in the first convolutional layers help capture local and low-level features and patterns. These are then combined in the next layers to extract higher-level ones. The final layers of a CNN are usually fully connected for making predictions based on the features learnt. 

\subsubsection{Recurrent Neural Networks (RNNs) and Its Variants}
RNNs are a specialised form of neural networks with recurrent connections that are well adapted to process sequential or time-series data \cite{das2023recurrent}, which can be arbitrarily long. RNNs and their variants can be used with different numbers of input and output tokens. They are especially useful in tasks related to natural language processing, e.g.\ machine translation, sentiment classification and image captioning, because text is sequential. The key element of RNNs is the \emph{hidden state}, which serves as a form of memory. The hidden state $\mathbf{h}_t$ at time step $t$ is calculated by applying an activation function $\sigma$ to a linear combination of the current input $\mathbf{x}_t$ and the hidden state $\mathbf{h}_{t-1}$ at the previous time step: \begin{equation}
    \mathbf{h}_t = \sigma(\mathbf{W}_{h} \mathbf{h}_{t-1} + \mathbf{W}_{x} \mathbf{x}_t + \mathbf{b}_{h}),
\end{equation}
where $\mathbf{W}_{h}$, $\mathbf{W}_{x}$ and $\mathbf{b}_{h}$ are parameters shared across all time steps. This leads to the vanishing gradient problem. If some weights are small, the repeated use of the chain rule in computing gradients will raise the weights to a power proportional to the number of time steps, hence causing the gradients to vanish. Therefore, early inputs no longer contribute much to predictions in the future. 

Gated Recurrent Units (GRUs) and long short-term memory (LSTM) networks are variants of RNNs which can better handle long-term dependencies. They achieve this with \emph{gates}. In simple terms, gates decide which information to be passed on by adding and removing different information. LSTMs maintain the cell state in addition to the hidden state. These extensions to vanilla RNNs allow relevant information further in the past to be kept for the future. 

The output of each cell of an RNN or its variant is some function of the hidden state at that time step. The number of outputs depends on the application. For example, classification for depression only requires one output at the last time step. 
\end{comment}

\subsection{Overview of ADD}
ADD generally refers to the task of determining whether an individual has depression or not without humans involved in the decision-making process. The input can be handcrafted features or raw data. The study of ADD started in 2009 \cite{ADD_first}. In that earliest work, Cohn et al.\ trained a support vector machine (SVM) classifier using features based on facial expressions and a logistic regression classifier with pitch and response latency as input features. They achieved an accuracy of 79\% for both models. Since then, more research on ADD has been carried out and performance has improved. 

The study of ADD is diverse, involving different types of data as well as DL and traditional ML techniques. In terms of data modality, there are two typical approaches \cite{depr_bipolar_review}. The first category makes use of physiological signals such as EEG \cite{eeg_depr_first}, electrocardiogram (ECG) \cite{6107702} and functional magnetic resonance imaging (fMRI) \cite{ROSA2015493}. More works focus on indirect behaviour cues of depression, e.g.\ in speech, text, movement, facial expressions, social interaction, etc. The data involved include text, audio, video, image and time series. The use of social media data is common because of its huge volume and diversity \cite{Islam, Shen}. 
%For instance, Islam et al.\ \cite{Islam} focused on text-based features such as linguistic style, sentiment and temporal focus, while Shen et al.\ \cite{Shen} also considered non-text-based cues, such as avatar, social interaction and posting time distribution. 
The models used are varied, with SVMs, decision trees and CNNs being the most commonly used \cite{depr_bipolar_review, MH_ML_review, MH_ML_review_camb}. 

Depression is diagnosed based on the criteria listed in the Diagnostic and Statistical Manual of Mental Disorders (DSM) \cite{dsm5}. Some ADD studies used clinical diagnosis as the ground truth, while others relied on the scores of questionnaires. Two popular questionnaires, which were designed based on the fourth edition of the DSM, are the Beck Depression Inventory-II (BDI-II) \cite{BDI} and the nine-item depression module of the Patient Health Questionnaire (called PHQ-9) \cite{PHQ-9}. The scores of different questionnaires might have different meanings. For instance, BDI-II and PHQ-9 focus on the severity and duration of symptoms for depression respectively \cite{BDI, PHQ-9}. 




Many studies on ADD using EEG \cite{eeg_depr_first, DeprNet, Ay} formulated the problem as a binary classification problem because their goal was to decide whether a signal belonged to a depressed or non-depressed individual. Nevertheless, a few studies formulated the problem as a regression problem. For example, Jan et al.\ \cite{depr_score_pred} used features based on facial and vocal expressions to predict BDI scores. 
%
One problem of many EEG-based studies is that the datasets are not publicly available. This undermines the reproducibility of results. 

\section{Fairness in ML}
\label{sec:ml_fairness}
For this section, we 
%begin with some terminology and notation that will aid understanding of later content. Consider 
adopt a generic binary classification approach. The input variable is $X$ taking values of $\mathcal{X}$ and the target variable is $Y$ with range $\mathcal{Y}$ = \{0, 1\}. $Y = 1$ is called the positive class and $Y = 0$ is called the negative class. Each individual has an associated sensitive attribute $S$, which is based on demographics that we want the predictions to be fair with respect to. If $S$ is a binary random variable, we refer to the group that is better represented in the data (majority group) by $s_1$ and the group that is underrepresented (minority group) by $s_0$. A classifier is a function $f: \mathcal{X} \rightarrow [0, 1]$ parameterised with $\theta$ that estimates the probability of belonging to the positive class. The prediction is $\hat{Y}$, which is 1 if $f(X) \geq 0.5$ or 0 otherwise. Performance is evaluated based on the target and prediction (see Table \ref{tab:metrics} for examples).

\begin{table}[h]
    \footnotesize
    \centering
    \begin{tabular}{c|c|c}
         & $\hat{y}=1$ & $\hat{y}=0$  \\
         \hline
         $y=1$ & true positive rate (TPR) & false negative rate (FNR) \\
         \hline
         $y=0$ & false positive rate (FPR) & true negative rate (TNR)
    \end{tabular}
    \emph{\caption{Performance metrics with the form $P(\hat{Y}=\hat{y}|Y=y)$}
    \label{tab:metrics}}
\end{table}

In this section, we describe fairness across groups decided by a \textbf{binary sensitive attribute}. The notion of fairness should be \emph{oblivious} \cite{eq_opp}, meaning it should depend only on the joint distribution of the target $Y$, prediction $\hat{Y}$ and sensitive attribute $S$. This allows the evaluation of fairness without interpreting individual features in $X$ or analysing the functional form of the classifier. This notion also fits with many fairness definitions in the literature. 
\subsection{Fairness Criteria, Definitions and Metrics}
\label{sec:fairness_def}
%Still, there are many ways to define fairness obliviously. 
There are three main criteria for fairness, namely independence, separation and sufficiency \cite{fairness_book}. Most fairness definitions are either equivalent or relaxed versions of one of these criteria. 
\begin{definition}
    Random variables $(\hat{Y}, S)$ satisfy \emph{independence} if they are independent.
\end{definition}
\begin{definition}
    Random variables $(\hat{Y}, S, Y)$ satisfy \emph{separation} if $\hat{Y}$ and $S$ are conditionally independent given Y. 
\end{definition}
\begin{definition}
    Random variables $(\hat{Y}, S, Y)$ satisfy \emph{sufficiency} if $Y$ and $S$ are conditionally independent given $\hat{Y}$. 
\end{definition} 

Now we introduce some of the most popular fairness definitions and their corresponding metrics. 
\subsubsection{Statistical Parity}
A classifier satisfies \emph{statistical parity}, or \emph{demographic parity} \cite{stat_parity}, if $\hat{Y}$ and $S$ are independent. In other words, \begin{equation} P(\hat{Y}=1|S=s_0) = P(\hat{Y}=1|S=s_1).
\end{equation}
This can be measured with $\mathcal{M}_{SP}=\frac{P(\hat{Y}=1|S=s_0)}{P(\hat{Y}=1| S=s_1)}$, which is called \emph{disparate impact} (DI) in the literature \cite{DI}. 

One characteristic, but also a limitation, of statistical parity is that it does not depend on the ground truth labels. This can be overcome with the following definitions which allow the predictions to be correlated with the sensitive attributes. 

\subsubsection{Equalised Odds and Equal Opportunity} 
A classifier satisfies \emph{equalised odds} \cite{eq_opp} if $\hat{Y}$ and $S$ are conditionally independent given $Y$, that is, if $(\hat{Y}, S, Y)$ satisfy separation. This means it has to satisfy \begin{equation} P(\hat{Y}=1|Y=y, S=s_0) = P(\hat{Y}=1|Y=y, S=s_1), y \in \{0, 1\}.
\end{equation}
This can be measured with $\mathcal{M}_{EOdd}=\frac{P(\hat{Y}=1|Y=0, S=s_0)}{P(\hat{Y}=1|Y=0, S=s_1)}$ and $\mathcal{M}_{EOpp}=\frac{P(\hat{Y}=1|Y=1, S=s_0)}{P(\hat{Y}=1|Y=1, S=s_1)}$ combined. 

The constraints for $y = 1$ and $y = 0$ require that the TPR and FPR (hence TNR) be equal across both demographic groups respectively. Good performance on the majority group only is not sufficient for equalised odds. 

There is a relaxation of equalised odds called {equal opportunity} \cite{eq_opp} that only enforces the constraint for $y = 1$. A binary classifier satisfies \emph{equal opportunity} if $\hat{Y}$ and $S$ are independent conditioned on $Y=1$, that is, \begin{equation} P(\hat{Y}=1|Y=1, S=s_0) = P(\hat{Y}=1|Y=1, S=s_1).
\end{equation}
The corresponding metric is $\mathcal{M}_{EOpp}$. 

\subsubsection{Equal Accuracy}
A classifier satisfies \emph{equal accuracy}, or \emph{overall accuracy equality} \cite{eq_acc}, if the accuracy is the same across all demographic groups. That is, \begin{equation}
    P(\hat{Y}=Y|S=s_0) = P(\hat{Y}=Y|S=s_1).
\end{equation}
This can be measured by $\mathcal{M}_{EAcc} = \frac{P(\hat{Y}=Y|S=s_0)}{P(\hat{Y}=Y|S=s_1)}$.

Equal accuracy can be treated as another relaxation of equalised odds. Instead of enforcing the same TPR and TNR for both groups, equal accuracy just requires their sum to be equal. 

Although equal accuracy is less common than the other definitions mentioned, it is still useful, especially when the overall accuracy is also provided. This gives an idea of the difference in performance of the classifier on the two groups. 

\subsubsection{Conditional Use Accuracy Equality and Predictive Parity}
A binary classifier satisfies \emph{conditional use accuracy equality} \cite{eq_acc} if both groups have the same probability of a positively predicted sample to belong to the positive class (called \emph{positive predictive value} (PPV)) and probability of a negatively predicted sample to belong to the negative class (called \emph{negative predictive value} (NPV)), that is, \begin{equation}
    P(Y=y|\hat{Y}=y, S=s_0) = P(Y=y|\hat{Y}=y, S=s_1), y \in \{0, 1\}.
\end{equation}
This is equivalent to saying that $(\hat{Y}, S, Y)$ satisfy sufficiency. This can be measured with 
$\mathcal{M}_{EPPV}=\frac{P(Y=1|\hat{Y}=1, S=s_0)}{P(Y=1|\hat{Y}=1, S=s_1)}$ and $\mathcal{M}_{ENPV}=\frac{P(Y=0|\hat{Y}=0, S=s_0)}{P(Y=0|\hat{Y}=0, S=s_1)}$ combined. 

There is a relaxation of conditional use accuracy equality called {predictive parity} \cite{predictive_parity} that only enforces the constraint for $y = 1$. A binary classifier satisfies \emph{predictive parity} if both groups have the same PPV, that is, \begin{equation}
    P(Y=1|\hat{Y}=1, S=s_0) = P(Y=1|\hat{Y}=1, S=s_1).
\end{equation}
The corresponding metric is $\mathcal{M}_{EPPV}$. 

\subsection{Bias Mitigation Strategies}
To mitigate bias, the simplest idea might be \emph{fairness through unawareness}, which means not using the sensitive attribute $S$ as a feature for prediction \cite{FTU}. However, this is usually inadequate because other input features might be correlated with $S$ and the classifier can infer this information to make its predictions. There are more involved techniques that approach bias mitigation at the data level. These are known as \emph{pre-processing} methods. There also exist \emph{in-processing} and \emph{post-processing} methods which aim to mitigate bias by modifying model training or the predictions themselves respectively. Figure \ref{fig:pipeline} provides an overview of bias mitigation at the pre-, in- and post-processing stages. In the following, we briefly describe some typical bias mitigation approaches under each of these three families \cite{bias_survey,info_theory, fairness_vis&lang_survey,bias_mit_survey,fairness_review}. 

\begin{figure}[h]
    \centering
    \includegraphics[width=1\columnwidth]{Pipeline.png}
    \emph{
    \caption{A simplified ML pipeline. The highlighted components indicate how bias is typically mitigated at the pre-, in- and post-processing stages.}
    \label{fig:pipeline}}
\end{figure}

\subsubsection{Pre-processing}
Pre-processing methods aim to eliminate bias at the earliest possible stage of the ML pipeline. They change the data distribution to remove bias in the training data \cite{fairness_review}. No data change is needed at inference time. Here are some common approaches. 
\begin{itemize}
    \item \emph{Relabelling}: The ground truth labels of some training examples are changed. To reduce the drop in accuracy, these examples are typically close to the decision boundary. One common purpose of relabelling is to ensure the same distribution of classes across demographic groups \cite{massaging}.
    \item \emph{Resampling}: Training examples are added or removed to produce a more balanced dataset \cite{massaging2}. 
    \item \emph{Feature perturbation}: This involves the addition, modification or removal of features of training examples \cite{DI, 3_naive_bayes}. 
    \item \emph{Fair representation}: The goal of this technique is to learn a new representation of the data that removes information related to the sensitive attribute while retaining as much information as possible. The classifier then makes predictions in this new representation space \cite{fair_repr}. 
\end{itemize}

\subsubsection{In-processing}
In-processing methods eradicate bias by directly changing the training procedure. This allows finer control of the performance-fairness balance when compared to pre-processing methods. However, resource constraints might make in-processing bias mitigation infeasible. Some in-processing methods adopt a multi-step approach, which allows unfair models to be fixed without retraining them from scratch \cite{fairness_vis&lang_survey}. We outline three common approaches under this category. 
\begin{itemize}
    \item \emph{Optimisation}: The common goal of different ML algorithms is to optimise some loss function. Therefore, incorporating fairness into the optimisation process is a widely applicable bias mitigation technique. This can be done by adding fairness constraints to the original constrained optimisation problem. An alternative is to add a regularisation term, just like L2 norm, to the loss function. This is particularly useful for gradient-based approaches \cite{reg1, reg2}. 
    \item \emph{Adversarial}: The adversarial approach attempts to train the classifier and an adversary simultaneously with the goals of maximising the accuracy of the classifier and minimising the ability of the adversary to predict the sensitive attribute. This helps train a classifier that does not use the sensitive attribute when making predictions \cite{adversarial}. 
    \item \emph{Compositional}: Instead of training a single model, compositional methods train multiple models which are combined in some way. For example, one model can be trained for each demographic group specified by the sensitive attribute \cite{3_naive_bayes}. 
\end{itemize}

\subsubsection{Post-processing}
Post-processing methods are performed after training is complete. It treats the trained model as a black box and makes the final predictions only using the sensitive attributes and output probabilities of the classifier \cite{bias_survey}. This makes it applicable to more types of models than pre-processing or in-processing methods. However, unlike the other two families, post-processing methods require access to sensitive attributes at inference time, which are not always available in real-world applications.
%, \hl{and use them explicitly}. 
The literature is less consistent regarding the categorisation of post-processing methods \cite{info_theory, fairness_vis&lang_survey,bias_mit_survey} so we do not provide one. 

\subsection{ML Fairness for MH Analysis and Depression Detection}
Research in ML fairness for MH analysis has been limited. Zanna et al.\ \cite{Zanna} proposed a multitask learning-based bias mitigation method for anxiety prediction using ECG and showed that it can improve fairness across different binary demographic attributes in terms of statistical parity and equalised odds better than a standard reweighing approach, although there was a drop in performance. Park et al.\ \cite{phone} investigated gender fairness for mental health assessment using phone-based data and showed that a pre-processing technique called DI remover \cite{DI} can improve some fairness metrics. 

Few researched ML fairness and bias mitigation for depression detection \cite{aguirre, postpartum}. 
%Aguirre et al.\ \cite{aguirre} tried balancing Twitter datasets across gender and race (the demographic labels were inferred) and reported on a slight fairness improvement. Park et al.\ \cite{postpartum} demonstrated the effectiveness of reweighing in improving fairness across race without compromising accuracy for detection of postpartum depression. 
Even fewer works made use of sensor data: Bailey and Plumbley \cite{Bailey_Plumbley_2021} showed that gender bias for depression detection using mel-spectrogram features resulted in an overreporting of F1 score. They mitigated the bias in the dataset using data redistribution but did not report any fairness metrics. Cheong et al.\ \cite{jiaee} investigated gender fairness for the detection of MH diseases, mainly depression. They found that pre-processing worked best at improving fairness for depression detection based on motor activity, but all methods failed at mitigating bias for detection using vlog data. 

Table \ref{tab:related_work} summarises existing work using sensor data and compares this work with those. Apart from the differences in data modality, our work and existing work differ in other ways. We attempt bias mitigation at all three stages, just like what Cheong et al.\ \cite{jiaee} did, but explore more methods. Instead of focusing on a single dataset or model, or training each model using just one dataset, we train different models using multiple datasets separately to give a more comprehensive discussion. 

\begin{table}[h]
    \centering
    \scalebox{0.9}{
    \hspace*{-1cm}\begin{tabular}{lccccccccccc}
        Authors & Year & Modality & D & M & Pre & In & Post & SP & EOpp & EOdd & EAcc \\ \hline
        % Aguirre et al. \cite{aguirre} & 2021 & ? & 2 & 1 & 1 & -- & -- & \cross & \tick & \tick & \cross \\
        % Park et al. \cite{postpartum} & 2021 & ? & 1 & 3 & 2 & 1 & -- & \tick & \tick & \cross & \cross \\
        Bailey and Plumbley \cite{Bailey_Plumbley_2021} & 2021 & Audio-visual & 1 & 2 & 1 & -- & -- & \cross & \cross & \cross & \cross \\
        Zanna et al.\ \cite{Zanna} & 2022 & Physiological & 1 & 1 & -- & 2 & -- & \tick & \cross & \tick & \cross \\
        \multirow{2}{*}{\centering Cheong et al. \cite{jiaee}} & \multirow{2}{*}{\centering 2023} & Audio-visual, & \multirow{2}{*}{\centering 3} & \multirow{2}{*}{\centering 2} & \multirow{2}{*}{\centering 1} & \multirow{2}{*}{\centering 1} & \multirow{2}{*}{\centering 1} & \multirow{2}{*}{\centering \tick} & \multirow{2}{*}{\centering \tick} & \multirow{2}{*}{\centering \tick} & \multirow{2}{*}{\centering \tick} \\ 
        & & motor activity \\ \hline
        Present work & 2024 & Physiological & 3 & 3 & 2 & 2 & 1 & \tick & \tick & \tick & \tick
    \end{tabular}\hspace*{-1cm}}
    \emph{
    \caption{Overview of studies on ML fairness for MH analysis and depression detection using sensor data. \emph{Abbreviations: D: Number of datasets. M: Number of distinct model architectures. Pre/In/Post: Number of pre-/in-/post-processing bias mitigation methods. SP: Statistical parity. EOpp: Equality of opportunity. EOdd: Equalised odds. EAcc: Equal accuracy. 
    %Empty cells indicate not being used.
    }}
    \label{tab:related_work}}
\end{table}

\chapter{Methodology}
\label{chap:methodology}
\emph{This chapter starts with a formulation of the research problem, then covers the performance and fairness metrics used. It also describes the bias mitigation methods utilised, in particular the proposed regularisation-based method.}

\section{Problem Formulation}
Building on top of the notation used in Section \ref{sec:ml_fairness}, we formulate depression detection using EEG data as a binary classification problem as follows: we are provided with a sequence of examples ($\mathbf{x}_i, y_i, z_i$) that have undergone pre-processing and feature extraction (if applicable). Tensor $\mathbf{x}_i \in \mathcal{X}$ represents information such as EEG signal or brain asymmetry image about an individual. The corresponding label is $y_i \in \mathcal{Y} = \{0, 1\}$. A depressed individual has a positive label $y_i = 1$ and a healthy individual has a negative label $y_i = 0$. The corresponding gender is $z_i \in $ \{\texttt{male}, \texttt{female}\}. Depending on the context, the minority group might be different. The dataset $D = \{(\mathbf{x}_i, y_i)\}_i$ is used to train a classifier $f: \mathcal{X} \rightarrow [0, 1]$ parameterised with $\theta$. As usual, the classification threshold is 0.5. The prediction for $\mathbf{x}_i$ is denoted by $\hat{y}$ and the predicted probability for it to be assigned to a class $c$ is denoted as $p(c|\mathbf{x}_i)$. The goal of training is to minimise the cross entropy loss, which is defined as \begin{equation}
    \mathcal{L}_{CE}(\mathbf{x}_i, y_i) = - y_i \log f(\mathbf{x}_i) - (1 - y_i) \log (1 - f(\mathbf{x}_i)) \label{eq:cross_entropy}
\end{equation}
for one training example $(\mathbf{x}_i, y_i)$. Note that $f(\mathbf{x}_i) = p(c = 1|\mathbf{x}_i)$. 

The reasons for choosing binary classification instead of regression are: 
\begin{itemize}
    \item this is a common approach in previous studies \cite{eeg_depr_first, DeprNet, Ay}; 
    \item it is easier to understand and interpret the performance metrics; and 
    \item modelling the task as a regression problem requires some real-valued score as the ground truth, but the meaning of depression scores is not standardised because of different depression questionnaires used \cite{BDI, PHQ-9}, and some studies do not collect this information. 
\end{itemize}

\section{Metrics}
%In this section, we introduce the performance and fairness metrics used. 

\subsection{Performance Metrics}
\label{sec:perf_metrics}
To facilitate the comparison of results, we choose to report the performance metrics commonly used in papers on ADD using EEG. These include metrics that are popular in general ML papers, including accuracy, precision and F1 score, as well as sensitivity and specificity. 
%Sensitivity and specificity are commonly used in medical and health-related applications. They are different ways to evaluate clinical tests for diseases. \emph{Sensitivity} refers to the ability of a test to correctly identify individuals carrying the disease. On the other hand, \emph{specificity} refers to the ability to correctly classify healthy individuals as not having the disease. Mathematically, sensitivity is just another name for recall or TPR, and specificity is another name for TNR. Sensitivity and specificity are inversely proportional, meaning as one increases, the other decreases \cite{sens&spec}.



\subsection{Fairness Metrics}
\label{sec:fair_metrics}
A binary classifier cannot satisfy all three criteria under reasonable assumptions such as $\hat{Y}$ not being independent of $Y$ and $Y$ not being independent of $S$ \cite{fairness_book}. The first assumption holds for our case because a reasonable classifier has different probabilities of predicting the positive class when fed with a signal from a depressed individual and a non-depressed individual. The second assumption holds because EEG signals are correlated with gender (recall Section \ref{sec:eeg}). Therefore, we concentrate on one criterion. We choose separation since it is an intuitive yet powerful notion of fairness. We avoid independence because it requires a classifier to classify the same percentage of individuals as depressed for both demographic groups, even if depression is around 50\% more prevalent in females than in males worldwide according to the WHO \cite{base_rate}. As a result, we evaluate fairness using $\mathcal{M}_{EOpp}$, $\mathcal{M}_{EOdd}$ and $\mathcal{M}_{EAcc}$, but keep $\mathcal{M}_{SP}$ as a reference. (Metrics are defined in Section \ref{sec:fairness_def}.)

A classifier is perfectly fair with respect to a certain notion if the corresponding metric equals 1. For practical purposes, the constraints are relaxed. If the metric falls between 0.8 and 1.2, the classifier is considered acceptably fair. These bounds conform to the literature \cite{Zanna} and relate to the ``80\% rule” in disparate impact law \cite{DI}. Note that for a classifier to be acceptably fair concerning equalised odds, $\mathcal{M}_{EOdd}$ and $\mathcal{M}_{EOpp}$ both have to fall in the specified range. 

\section{Existing Bias Mitigation Methods}
\label{sec:existing_methods}
Many bias mitigation methods have been proposed. However, not all methods apply to our task because some only work for a particular data modality, data type (discrete or continuous), fairness definition, model or problem formulation. We introduce five methods that are particularly suited for our purposes and span all three stages of the ML pipeline.
%as illustrated in Figure \ref{fig:pipeline}
% Note that the methods massaging \cite{massaging} and Reject Option based Classification \cite{ROC} require the definition of a desirable label or class. This refers to the depressed class because we are interested in detecting depression. 

\subsection{Pre-processing}
We make use of two pre-processing methods that change the dataset distribution differently to reduce bias. We wish to emphasise that these changes only happen at training but not at inference time. 
\subsubsection{Data Augmentation}
We employ a data augmentation technique termed \emph{mixup} that was designed by Zhang et al.\ \cite{mixup} because this technique is simple yet effective and can work with different types of data, including images and waveforms. Under the assumption that linear interpolations of feature vectors result in linearly interpolated targets, a new training example $(\mathbf{x}', y')$ is generated from two randomly drawn examples $(\mathbf{x}_i, y_i)$ and $(\mathbf{x}_j, y_j)$ with $i \neq j$ by \begin{gather}
    \mathbf{x}' = \lambda \mathbf{x}_i + (1 - \lambda)\mathbf{x}_j, \\
    y' = \lambda y_i + (1 - \lambda)y_j,
\end{gather}
where $\lambda \sim \mathrm{Beta}(\alpha, \alpha)$ for some hyperparameter $\alpha$ that controls the strength of interpolation. Note that $\lambda \in [0, 1]$ because of the beta distribution. %The equations above preserve the relation between features and targets. 
We generate these examples for the minority group so that the resulting dataset is balanced across gender. Although $y'$ might not be an integer, the loss can still be calculated as the cross entropy between the target and predicted distributions using Equation (\ref{eq:cross_entropy}). Regarding the choice of $\alpha$, the authors found that the performance improved when $\alpha \in [0.1, 0.4]$. After testing different values of $\alpha$ in this interval, we pick $\alpha = 0.4$ which gives the best results. 

\subsubsection{Massaging}
To allow comparison of data augmentation with another type of pre-processing, we implement massaging which is popular \cite{bias_mit_survey} among relabelling techniques. This was proposed by Kamiran and Calders \cite{massaging}, initially for na\"ive Bayes but later extended to other classifiers \cite{massaging2}. For a dataset $D$, the favoured community ($s_\mathrm{fav}$) refers to the demographic group with a higher probability of belonging to the favourable class $c_+$, and the other group is called the deprived community ($s_\mathrm{dep}$). Since we are interested in detecting depression, $c_+$ refers to the depressed class. The discrimination of $D$, which is a measure of how biased the dataset is, is defined as \begin{equation}
    disc(D) = P(Y=c_+|S=s_\mathrm{fav}) - P(Y=c_+|S=s_\mathrm{dep}).
\end{equation}
The goal of massaging is to produce a modified dataset with minimal discrimination by relabelling the same number of instances from the favoured community with a favourable label and instances from the deprived community with an unfavourable label. Based on simple calculations, the number of relabelled pairs needed is \begin{equation}
    m = \lceil disc(D) \times P(S=s_\mathrm{fav}) \times P(S=s_\mathrm{dep}) \times |D| \rceil.
\end{equation}
After relabelling, the distribution of classes is unchanged, but the class distribution is now the same across both genders, and the gender ratio is equal in both classes. 
To minimise the impact on performance, we relabel the examples that are considered closest to the class boundary, which are those with the lowest prediction probabilities for their ground truth class. We obtain these by training the classifiers using the original dataset and sorting the examples based on the prediction probabilities. After relabelling, we retrain the classifier using the modified dataset. 

\subsection{In-processing}
The original loss function for a batch $B$ is \begin{equation}
    \mathcal{L}(B) = \frac{1}{|B|} \sum_{(\mathbf{x}_i, y_i) \in B} \mathcal{L}_{CE}(\mathbf{x}_i, y_i). 
\end{equation}
We adopt two in-processing methods that change this loss function in different ways. 
\subsubsection{Reweighing}
Reweighing is an alternative to resampling \cite{massaging2}. It also calculates weights $\beta_i$ for each example, but the weights are directly incorporated into the loss function as follows: \begin{equation}
    \mathcal{L}_w(B) = \frac{1}{|B|} \sum_{(\mathbf{x}_i, y_i) \in B} \beta_i \, \mathcal{L}_{CE}(\mathbf{x}_i, y_i). 
\end{equation}

We choose these weights based on a scheme suggested by Calders et al.\ \cite{reweighing} that is effective and frequently used. According to their work, the weight for an example $(\mathbf{x}_i, y_i)$ with associated gender $z_i$ is \begin{equation}
    \beta_i = \frac{P(Y=y_i) \times P(S=z_i)}{P(Y=y_i \wedge S=z_i)} = \frac{P(Y=y_i)}{P(Y=y_i|S=z_i)}. 
\end{equation}
These weights are the same for each combination of gender and class. The distribution of weights is the same across genders and across classes. Since the weight-adjusted gender ratio is the same for both classes, the classifier cannot improve performance by associating each gender with a certain class. 

\subsubsection{Regularisation}
Broadly speaking, regularisation is the addition of a penalty term to the loss function to influence the training process and hence the final learnt model \cite{bishop1995neural}. We choose this method because it is powerful and can adapt to different purposes.
% For our purposes, the penalty term is used to control fairness. 
As mentioned in Section \ref{sec:fair_metrics}, we wish to enforce separation. This requires both groups to have equal TPRs and equal FPRs. We therefore design two regularisation terms to minimise the absolute difference in TPRs and FPRs of the two groups respectively. The principle is that when these differences are small, the fairness metrics will be close to 1. The idea behind these regularisation terms comes from Bechavod and Ligett \cite{reg1}, but we estimate the TPRs and FPRs using prediction probabilities instead of the predictions themselves because the probabilities are more informative. This estimation approach is similar to the work of Manisha and Gujar \cite{reg2}. Furthermore, unlike the mentioned works, we adopt a \textbf{two-stage} training approach that fine-tunes a trained model. Compared with retraining the model from scratch, this can achieve comparable or even better performance with fewer training epochs. For a batch $B$, we write $B_k$ for the instances in the group $s_k$. The estimated TPR for $s_k$ is \begin{equation}
    \mathrm{TPR}_k(B) = \frac{\sum_{(\mathbf{x}_i, y_i) \in B_k} y_i \, f(\mathbf{x}_i)}{\sum_{(\mathbf{x}_i, y_i) \in B_k} y_i}
\end{equation}
and the estimated FPR for the group $s_k$ is \begin{equation}
    \mathrm{FPR}_k(B) = \frac{\sum_{(\mathbf{x}_i, y_i) \in B_k} (1 - y_i) f(\mathbf{x}_i)}{\sum_{(\mathbf{x}_i, y_i) \in B_k} (1 - y_i)}
\end{equation}
We define the absolute difference between the estimated TPRs as \begin{equation}
    d_t(B) = |\mathrm{TPR}_0(B) - \mathrm{TPR}_1(B)|
\end{equation}
and similarly that between the estimated FPRs as \begin{equation}
    d_f(B) = |\mathrm{FPR}_0(B) - \mathrm{FPR}_1(B)|
\end{equation}
These difference terms are used to define the new loss function which is \begin{equation}
    \mathcal{L}_\mathrm{reg}(B) = \mathcal{L}(B) + \lambda_{EOpp} \, d_t(B) + \lambda_{EOdd} \, d_f(B),
\end{equation}
where $\lambda_{EOpp}$ and $\lambda_{EOdd}$ are hyperparameters. 

\subsection{Post-processing}
Due to the smaller number of variants of post-processing techniques and time constraints, we only choose one representative post-processing method that makes changes to the predicted labels. %The dataset and classifier remain unchanged. 

\subsubsection{Reject Option based Classification (ROC)}
We adopt an ROC method based on the work of Kamiran et al.\ \cite{ROC} since it has the advantages of being lightweight and only using the prediction probabilities for an instance to modify its predicted class. As the name suggests, this approach attempts to improve fairness by re-classifying ``rejected instances”, which are instances with prediction probabilities close to the classification threshold of 0.5. In more detail, we select a desirable label $c_+$ and some parameter $\tau$ satisfying $0.5 < \tau < 1$ to define a decision boundary (termed critical region): if $1 - \tau \leq p(c_+|\mathbf{x}_i) \leq \tau$, and the instance belongs to the minority group, then it is assigned to class $c_+$. Otherwise, the instance is classified using the original decision rule. The intuition behind this method is to give the minority group an advantage when the classifier is unsure about the predictions. For our case, the depressed class is of interest so $c_+ = 1$, and we choose $\tau = 0.6$ based on suggestions by the authors and empirical results. 



\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Method.png}
    \emph{\caption{An illustration of how the proposed method fits into the pipeline in the second stage of training.}
    \label{fig:new_method}}
\end{figure}

%\chapter{Experimental Setup}
\section{Experimental Setup}
\label{chap:setup}
\emph{This chapter introduces the datasets and models used for the experiments and describes how the models were implemented and trained using different datasets.}
\section{Datasets}
The inclusion criteria for datasets are as follows: they must consist of EEG data, be publicly available for reproducibility and contain sex attributes for fairness evaluation. We choose three commonly used datasets that meet these requirements. They are (1) MDD Patients and Healthy Controls EEG Data (New) \cite{data2}, (2) Multi-modal Open Dataset for Mental-disorder Analysis \cite{modma} and (3) EEG: Depression rest \cite{rest}. We will refer to them by Mumtaz, MODMA and Rest respectively. For comparability, all datasets contain resting-state EEG data. Since all datasets contain data acquired during eyes-closed (EC) conditions, but some do not have eyes-open (EO) data, we concentrate on EC data. Table \ref{tab:datasets} shows the number of individuals involved in each dataset, grouped by gender and label. For all three datasets, no standard train-test split was provided by the owners. 

\begin{comment}

\begin{table}[h]
    \centering
    \scalebox{0.9}
    {\begin{tabular}{c|ccc|ccc|ccc}
         & \multicolumn{3}{|c|}{\textbf{Mumtaz}} & \multicolumn{3}{|c|}{\textbf{MODMA}} & \multicolumn{3}{|c}{\textbf{Rest}} \\ \cline{2-10}
         & Male & Female & Total & Male & Female & Total & Male & Female & Total \\ \hline
         Depressed & 17 & 13 & 30 & 13 & 11 & 24 & 12 & 34 & 46 \\
         Healthy & 20 & 8 & 28 & 20 & 9 & 29 & 35 & 40 & 75 \\
         Total & 37 & 21 & 58 & 33 & 20 & 53 & 47 & 74 & 121
    \end{tabular}}
    \emph{\caption{Dataset distribution}
    \label{tab:datasets}}
\end{table}

\end{comment}

\vspace{-6pt}
\subsubsection{Mumtaz}
Data in this dataset were recorded using an EEG cap with 19 electro-gel sensors, placed according to the 10-20 system. Data collection was performed during EC and EO conditions for 5 minutes but we only use the EC data. The sampling rate is 256 Hz. %The dataset also contains event-related potential data which is unused. 
64 participants were recruited but the dataset only contains data from 58 individuals. 30 of them were diagnosed with depression based on DSM criteria. The rest were age-matched healthy controls. The dataset contains data from 37 males and 21 females so females are the minority \cite{mumtaz_paper}.

\subsubsection{MODMA}
The MODMA dataset consists of recordings of one spoken language experiment and several sets of EEG data from clinically depressed patients and matching healthy controls. We only utilise one set of EEG data collected with a 128-channel HydroCel Geodesic Sensor Net, which contains 5-minute-long EC resting-state EEG signals. The sampling rate is 250 Hz. Out of the 53 participants involved, 24 individuals were diagnosed with depression based on DSM criteria. The dataset contains data from 33 males and 20 females so females are the minority \cite{modma}. 

\subsubsection{Rest}
This dataset involves collecting resting-state EEG data with 64 Ag/AgCl electrodes using a SynAmps 2 system. The sampling rate is 500 Hz. We only use data from the first test run. % Not all participants received clinical interviews, 
The ground truth was based on BDI scores. 121 college-age participants were involved, with 46 belonging to the depressed group. The dataset contains data from 47 males and 74 females so males are the minority \cite{rest_paper}. This dataset was not used by the models introduced in the next section.
% \hl{so it can be used to test for generalisation of models across datasets.} 

\section{Models}
The inclusion criteria for models are as follows: the models must be trained using one of the three publicly available datasets and there should be clear documentation of how the models were implemented and trained so the results could be reproduced. It would be ideal if some source code is available. We focus on DL architectures because they have become popular but their fairness is under-investigated. 

The three algorithms chosen are Deep-Asymmetry \cite{Deep-Asymmetry}, gated temporal-separable attention network (GTSAN) \cite{GTSAN} and 1DCNN-LSTM \cite{1DCL}. For comprehensiveness, we deliberately choose algorithms that make use of different model architectures and process EEG data differently. We briefly describe these algorithms in the following paragraphs. 

\subsubsection{Deep-Asymmetry}
Kang et al.\ \cite{Deep-Asymmetry} proposed the Deep-Asymmetry method for depression detection using brain asymmetry. They utilised the Mumtaz dataset. EEG pre-processing steps included min-max normalisation per channel, noise removal through independent component analysis and partition into non-overlapping 4-second segments. For each frequency band (e.g. alpha), the relative power of each channel was calculated using Welch’s periodogram and Simpson’s method. The difference in relative power of each pair of channels (16 channels in total) was used to create a matrix-type image. These images were then fed into a CNN-based model with 3 convolutional layers. Table \ref{tab:model1} shows the architecture. Separate models were trained using images generated for the four different frequency bands. We only report results for the alpha band which has the best performance. Performance was evaluated using 5-fold cross-validation.



\subsubsection{GTSAN}
Yang et al.\ \cite{GTSAN} proposed the GTSAN model and trained it with the MODMA dataset. They first sliced the data into 1-second segments, then extracted the power spectral density features of different frequency bands before performing z-score standardisation on the features. The flattened feature vectors were fed into both a GRU and a network made up of separable and dilated causal convolutional layers. The outputs were passed to an attention layer followed by a fully connected layer. Tables \ref{tab:model2a} and \ref{tab:model2b} summarise the architecture. Performance was evaluated using a test set. 





\subsubsection{1DCNN-LSTM}
Mumtaz and Qayyum \cite{1DCL} implemented two models and we adopt the second one, which has both one-dimensional convolutional layers and LSTM layers. Table \ref{tab:model3} shows the architecture. They utilised the Mumtaz dataset. Since EEG data in the dataset already had noise removed, the authors only performed min-max normalisation. 1-second segments of 19-channel EEG signals were directly fed into the model. Performance was evaluated using a test set. This model has an architecture similar to one of the best-performing models by Ay et al.\ \cite{Ay}, which was trained using private datasets.


\section{Implementation and Training Details}
\label{sec:implm_training}

In this section, we describe how the models were implemented and trained. For each algorithm, we first mention how we tried reproducing the results from existing work with the same dataset, using the hyperparameters given in the paper or source code. We then state how we retrained the model with other datasets. We left the pre-processing pipeline and model structure unchanged but used hyperparameters tuned via manual or random search. The last part of the section is related to bias mitigation.

We used Python 3.11, Tensorflow 2.15.0 and Keras 2.15.0 for the implementation. The authors of all three algorithms released code snippets that included important processing steps, model architectures and training hyperparameters but these were not fully functional code. We removed redundant parts, fixed bugs, added pre-processing code and adapted the code as needed for different datasets. All authors provided dataset splits but did not utilise subject-independent training. We adhered to these specifications.  


\subsubsection{Deep-Asymmetry}
To reproduce results for the Mumtaz dataset, we trained the model for 10 epochs using an Adam optimiser with learning rate initialised as 0.0001. The mini-batch size was 75 and the dropout rate was 0.25. 

For the other two datasets, a different number of electrodes and/or different electrode placement systems were used. We produced a one-to-one mapping between electrode names and then selected the 16 channels needed. The sampling rate was taken care of during the calculation of relative powers. 

The previous mini-batch size and dropout rate worked well for both datasets. For MODMA, we trained the model for 50 epochs using an Adam optimiser with learning rate initialised as 0.00002. We also added L2 regularisation of strength 0.01 to the dense layer. For the Rest dataset, the learning rate of Adam was 0.00005 and the number of epochs was 20. 

\subsubsection{GTSAN}
To reproduce results for MODMA, we trained the model for 150 epochs with early stopping using an RMSprop optimiser with learning rate initialised as 0.002. The mini-batch size was 128 and the dropout rate was 0.2. 

The authors provided a train/test split of 8:2. For hyperparameter optimisation, we used 80\% of the training set for training and the rest for validation. For evaluation, we trained the model using the whole training set. 

For the Mumtaz dataset, the optimal settings include an RMSprop optimiser with learning rate initialised as 0.01, dropout rate of 0.2, batch size of 128, training time of 150 epochs (with early stopping), reduction of model size by half and addition of L2 regularisation of strength 0.002 to all layers. 

For the Rest dataset, we tried adjusting all possible hyperparameter settings, including the ones mentioned above, the type of optimiser (e.g.\ Adam), activation functions (e.g.\ ELU), hyperparameters for the optimiser and the number of dropout layers. However, the performance was still poor. We therefore did not conduct further experiments but will briefly discuss the implications in Section \ref{sec:discussion}. 

\subsubsection{1DCNN-LSTM}
To reproduce results for the Mumtaz dataset, we trained the model for 20 epochs using an Adam optimiser with learning rate initialised as 0.0004. The mini-batch size was 50 and the dropout rate was 0.5. 

The other two datasets had different sampling rates so they were resampled to 256 Hz at the start. Besides, the number of channels was different. We checked that the performance would be too strong if all channels were used. For comparability of performance, we only kept the corresponding 19 channels, just like what we did for the Deep-Asymmetry algorithm. 

The authors provided a train/val/test split so we used the specified validation set for hyperparameter tuning. For MODMA, we trained the model for 30 epochs using an Adam optimiser with learning rate initialised as 0.00004. The mini-batch size was 50 and the dropout rate was 0.2. For the Rest dataset, we trained the model for 30 epochs using an Adam optimiser with learning rate initialised as 0.0004. The mini-batch size was 128 and the dropout rate was 0.3. We also added L2 regularisation of strength 0.001 to the convolutional and LSTM layers. 

\section{Bias Mitigation}
We calculated our own fairness metrics based on descriptions in Section \ref{sec:fairness_def} and implemented bias mitigation methods as described in Sections \ref{sec:existing_methods} and \ref{sec:new_method}. Regarding the proposed method, since keeping $\gamma_{EOpp}$ and $\gamma_{EOdd}$ equal usually gives better results, we replace them with the single hyperparameter $\gamma$ in the rest of the discussion. Table \ref{tab:hyperpara_new} shows the hyperparameters used for the original and proposed regularisation methods. 

\begin{table}[]
    \centering
    \footnotesize
    \addtolength{\tabcolsep}{-1mm}
    \begin{tabular}{ll|cc|ccc}
         & & \multicolumn{2}{|c|}{Original} & \multicolumn{3}{|c}{Proposed} \\ 
         & & $\lambda_{EOpp}$ & $\lambda_{EOdd}$ & $\lambda_{EOpp}$ & $\lambda_{EOdd}$ & $\gamma$ \\ \hline
         \multirow{3}{*}{\centering Deep-Asymmetry} & Mumtaz & 2.0 & 2.0 & 1.5 & 2.5 & 20.0 \\
         & MODMA & 2.0 & 0.5 & 2.0 & 2.0 & 20.0 \\
         & Rest & 2.0 & 0.5 & 3.0 & 2.0 & 20.0 \\ \hline
         \multirow{2}{*}{\centering GTSAN} & Mumtaz & 2.0 & 2.0 & 1.0 & 1.0 & 20.0 \\
         & MODMA & 2.0 & 2.0 & 0.4 & 0.4 & 20.0 \\ \hline
         \multirow{3}{*}{\centering 1DCNN-LSTM} & Mumtaz & 10.0 & 5.0 & 2.5 & 5.0 & 10.0 \\
         & MODMA & 20.0 & 5.0 & 0.9 & 1.0 & 20.0 \\
         & Rest & 2.0 & 2.0 & 2.0 & 2.0 & 20.0 \\
    \end{tabular}
    \emph{\caption{Hyperparameter choice for two regularisation methods}
    \label{tab:hyperpara_new}}
\end{table}

%\chapter{Results and Analysis}
\section{Results and Analysis}
\label{chap:results}
\emph{This chapter describes the results of the experiments, which were carried out using the methodology and experimental setup detailed in the previous two chapters, answers the RQs and discusses the results.}
\section{Experimental Results}
\label{sec:results}

%Before answering the three RQs, we first briefly describe the performance of the algorithms in depression detection.
% with reference to Table \ref{tab:performance_results}. 
In this section, we describe the results for each dataset in the following order: performance of algorithms, bias of algorithms, bias mitigation using existing methods and bias mitigation using the proposed method. The last three items are related to the three RQs stated in Section \ref{sec:RQ} respectively. We summarise the results and give an overall answer to each RQ in the next section. 

\subsection{Mumtaz}
We start with the results for Mumtaz with reference to Table \ref{tab:dataset1}.

\begin{table}[t]
    \scriptsize
    \centering
    %\captionsetup{font=scriptsize}
    %\scalebox{0.62}{
    \begin{tabular}{ll|cccccc|c}
         %& & \multicolumn{7}{|c}{\textbf{Mumtaz}} \\ \cline{3-9}
         & & Base & Aug & Mas & RW & Reg & ROC & Reg+ \\ \hline
         \multirow{18}{*}{\centering \begin{sideways}\textbf{Deep-Asymmetry}\end{sideways}} & \multirow{2}{*}{\centering Accuracy} & 0.98 & \textbf{0.99} & 0.97 & 0.98 & 0.98 & \textbf{0.99} & 0.98 
\\
         & & ±0.00 & ±0.00 & ±0.00 & ±0.00 & ±0.00 & ±0.00 & ±0.00
\\
         & \multirow{2}{*}{\centering Sensitivity} & \textbf{0.99} & 0.98 & 0.97 & 0.98 & 0.98 & 0.98 & 0.97
\\
         & & ±0.00 & ±0.01 & ±0.01 & ±0.00 & ±0.0122 & ±0.0052 & ±0.0070 
\\
         & \multirow{2}{*}{\centering Specificity} &  0.9814 & 0.9898 & 0.9700 & 0.9714 & 0.9795 & \textbf{0.9902} & 0.9848 
\\
         & & ±0.0068 & ±0.0044 & ±0.0127 & ±0.0062 & ±0.0104 & ±0.0018 & ±0.0061 
\\
         & \multirow{2}{*}{\centering Precision} & 0.9828 & 0.9805 & 0.9721 & 0.9736 & 0.9810 & 0.9800 & \textbf{0.9856} 
\\
         & & ±0.0062 & ±0.0092 & ±0.0113 & ±0.0055 & ±0.0094 & ±0.0058 & ±0.0056 
\\
         & \multirow{2}{*}{\centering F1} & 0.9854 & \textbf{0.9858} & 0.9711 & 0.9781 & 0.9784 & \textbf{0.9858} & 0.9767 
\\
         & & ±0.0030 & ±0.0025 & ±0.0050 & ±0.0020 & ±0.0025 & ±0.0029 & ±0.0019 
\\ \cline{2-9}

         & \multirow{2}{*}{\centering $\mathcal{M}_{SP}$} & 1.3236 & 1.3265 & 1.2897 & 1.3130 & 1.3097 & 1.3345 & 1.3123 
\\
         & & ±0.1232 & ±0.1394 & ±0.1406 & ±0.1295 &  ±0.1316 & ±0.1219 & ±0.1250 
\\
         & \multirow{2}{*}{\centering $\mathcal{M}_{EOpp}$} & 0.9958 & \textbf{1.0000} & 0.9814 & 0.9944 & 0.9913 & 1.0010 & 0.9818 
\\
         & & ±0.0053 & ±0.0068 & ±0.0163 & ±0.0094 &  ±0.0112 & ±0.0055 & ±0.0115 
\\
         & \multirow{2}{*}{\centering $\mathcal{M}_{EOdd}$} & 0.8016 & 0.5879 & 0.8813 & 0.7732 & \textbf{0.9064} & 1.1886 & 0.8403 
\\
         & & ±0.6554 & ±0.3416 & ±0.7773 & ±0.5462 & ±1.0860 & ±1.0255 & ±0.6035 
\\
         & \multirow{2}{*}{\centering $\mathcal{M}_{EAcc}$} & 1.0030 & 1.0073 & \textbf{0.9981} & 1.0039 & 1.0020 & 1.0043 & 0.9895
\\
         & & ±0.0037 & ±0.0057 & ±0.0231 & ±0.0086 & ±0.0174 & ±0.0052 & ±0.0070 
\\ \hline
         
         \multirow{9}{*}{\centering \begin{sideways}\textbf{GTSAN}\end{sideways}} & Accuracy &  0.7787 & 0.7716 & 0.7299 & 0.7399 & 0.7213 & \textbf{0.7816} & 0.7069 
\\
         & Sensitivity & 0.8448 & 0.8193 & 0.7455 & 0.8601 & 0.7735 & \textbf{0.8728} & 0.7863 
\\
         & Specificity & 0.6931 & \textbf{0.7096} & \textbf{0.7096} & 0.5842 & 0.6535 & 0.6634 & 0.6040 
\\
         & Precision & 0.7812 & \textbf{0.7854} & 0.7690 & 0.7284 & 0.7433 & 0.7708 & 0.7203 
\\
         & F1 & 0.8118 & 0.8020 & 0.7571 & 0.7888 & 0.7581 & \textbf{0.8186} & 0.7518 
\\ \cline{2-9}

         & $\mathcal{M}_{SP}$ & 1.0523 & 1.0217 & 0.9292 & 1.0161 & 1.0255 & 1.1935 & 1.1364
\\
         & $\mathcal{M}_{EOpp}$ & 1.0320 & 0.9687 & 0.9337 & \textbf{1.0138} & 0.9177 & 1.1155 & 1.0379 
\\
         & $\mathcal{M}_{EOdd}$ & 0.4687 & 0.5457 & 0.3698 & 0.6102 & 0.9014 & 0.7933 & \textbf{1.0048}
\\
         & $\mathcal{M}_{EAcc}$ & 1.1489 & 1.0760 & 1.0789 & 1.1683 & \textbf{0.9892} & 1.1603 & 1.0665 
\\ \hline

         \multirow{9}{*}{\centering \begin{sideways}\textbf{1DCNN-LSTM}\end{sideways}} & Accuracy & \textbf{0.9956} & 0.9942 & 0.8891 & 0.9518 & 0.8569 & 0.9927 & 0.8744 
\\
         & Sensitivity & 0.9915 & 0.9915 & 0.9153 & 0.9181 & 0.9633 & 0.9915 & \textbf{0.9972} 
\\
         & Specificity & \textbf{1.0000} & 0.9970 & 0.8610 & 0.9879 & 0.7432 & 0.9940 & 0.7432
\\
         & Precision & \textbf{1.0000} & 0.9972 & 0.8757 & 0.9878 & 0.8005 & 0.9943 & 0.8059 
\\
         & F1 & \textbf{0.9957} & 0.9943 & 0.8950 & 0.9517 & 0.8744 & 0.9929 & 0.8914 
\\ \cline{2-9}
         & $\mathcal{M}_{SP}$ & 1.1159 & 1.1249 & 0.9331 & 0.9590 & 0.9462 & 1.1338 & 1.0508
\\
         & $\mathcal{M}_{EOpp}$ & \textbf{1.0008} & 1.0133 & 0.8923 & 0.8758 & 0.9087 & \textbf{1.0008} & 0.9921 
\\
         & $\mathcal{M}_{EOdd}$ & $\infty$ & 0.0000 & 0.6326 & 0.0000 & 0.7952 & $\infty$ & \textbf{0.9488} 
\\
         & $\mathcal{M}_{EAcc}$ & \textbf{1.0000} & 1.0088 & 0.9720 & 0.9385 & 0.9883 & 0.9911 & 1.0189
\\
    \end{tabular}%}
    \emph{\caption{Summary of performance and fairness results for the \textbf{Mumtaz} dataset. \emph{Abbreviations: Base: Baseline. Aug: Data augmentation. Mas: Massaging. RW: Reweighing. Reg: Regularisation. Reg+: Proposed method. Remarks: Bold values indicate the best results for each metric, except the reference metric $\mathcal{M}_{SP}$, across bias mitigation methods. The standard deviation across the 5 folds is provided for Deep-Asymmetry.}}
    \label{tab:dataset1}
    }
\end{table}

We describe the performance of models as shown in the ``Base" column. We successfully reproduced the results of the original paper \cite{Deep-Asymmetry} for Deep-Asymmetry. Our trained model had an accuracy of 0.9848, sensitivity of 0.9880 and specificity of 0.9814 while the paper reported an accuracy of 0.9885, sensitivity of 0.9915 and specificity of 0.9851. The results we obtained for 1DCNN-LSTM were also in line with the original work \cite{1DCL}, which omitted exact values. With additional shuffling of the training set, we even observed performance improvements. Overall, 1DCNN-LSTM had the best performance while GTSAN had the worst performance when trained with Mumtaz. There was a trade-off between sensitivity and specificity, with them either being the best or worst performance metric. Deep-Asymmetry and GTSAN performed best while 1DCNN-LSTM performed worst in terms of sensitivity.

We next describe the fairness results using the ``Base" column. All three algorithms are acceptably fair in terms of equal opportunity and equal accuracy because their $\mathcal{M}_{EOpp}$ and $\mathcal{M}_{EAcc}$ values lie between 0.8 and 1.2. However, only Deep-Asymmetry has $\mathcal{M}_{EOdd}$ within the 0.8--1.2 range. For GTSAN, the value is 0.4687, which suggests bias in favour of males. For 1DCNN-LSTM, $\mathcal{M}_{EOdd}$ is undefined because the denominator is 0 but the numerator is not. This can be interpreted as bias towards females. Among the three algorithms, 1DCNN-LSTM is the fairest in terms of the more relaxed equal opportunity and equal accuracy frameworks because $\mathcal{M}_{EOpp}$ and $\mathcal{M}_{EAcc}$ are very close to 1. However, it is the most biased in terms of the stricter equalised odds framework because $\mathcal{M}_{EOdd}$ is the most extreme. On the other hand, Deep-Asymmetry satisfies all three frameworks. Overall, 1DCNN-LSTM is the most biased and Deep-Asymmetry is the fairest. 

We now describe the results of bias mitigation using the five mentioned methods for each model. This is done by comparing the ``Base" column with the 5 columns following it. 

\textbf{Deep-Asymmetry} \quad Across all metrics, performance is comparable before and after carrying out data augmentation or ROC, while the performance drops slightly after performing other bias mitigation methods. $\mathcal{M}_{EOpp}$ and $\mathcal{M}_{EAcc}$ are more or less the same as before across all mitigations. Data augmentation and reweighing cause $\mathcal{M}_{EOdd}$ to fall below 0.8, making the model biased in favour of males. The other three methods cause $\mathcal{M}_{EOdd}$ to increase but remain below 1.2, meaning the model is still fair. This metric is closer to 1 when massaging or regularisation is performed. Overall, \textbf{regularisation} provides the best performance-fairness trade-off since it produces fairness metrics closest to 1 at a small cost of performance. 

\textbf{GTSAN} \quad Only massaging, reweighing and regularisation affect performance negatively. Different mitigation methods alter $\mathcal{M}_{EOpp}$ and $\mathcal{M}_{EAcc}$ in different directions, but none bring them out of the 0.8--1.2 range. All except massaging increase $\mathcal{M}_{EOdd}$ and reduce bias in favour of males, but only regularisation brings it within the fairness bounds. We conclude \textbf{regularisation} produces a fair model at a cost of performance. 

\textbf{1DCNN-LSTM} \quad Apart from data augmentation and ROC, all mitigation methods worsen performance in general, especially for massaging and regularisation. All methods other than data augmentation decrease $\mathcal{M}_{EOpp}$ and $\mathcal{M}_{EAcc}$ slightly, but no method brings them out of the 0.8--1.2 range. Only massaging and regularisation lead to non-zero and defined $\mathcal{M}_{EOdd}$, but the value is below 0.8. These two offer good but different performance-fairness trade-offs. \textbf{Massaging} outperforms regularisation across most performance metrics but has more bias towards females, while \textbf{regularisation} has better sensitivity and $\mathcal{M}_{EOdd}$ closer to the boundary 0.8. 

Overall, \textbf{regularisation} is the best in bias mitigation for Mumtaz as evidenced by the results of the three models.

Finally, we provide the results of bias mitigation with the improved regularisation approach (``Reg+" column) and compare it with the original regularisation approach (``Reg" column) and the method that gives the best performance-fairness trade-off. 

\textbf{Deep-Asymmetry} \quad Compared with the original approach, the new approach achieves similar performance across all metrics. The new approach decreases all three fairness metrics, but they still lie in the range 0.8--1.2, indicating fairness. Although $\mathcal{M}_{EOdd}$ is a bit further away from 1, its standard deviation is reduced, meaning the new approach helps reduce the variance of fairness when using different training data. 

\textbf{GTSAN} \quad Changing the regularisation approach causes a small performance drop across all metrics except sensitivity. Although the model already satisfies all three fairness definitions after regularisation, the new approach brings $\mathcal{M}_{EOpp}$ and $\mathcal{M}_{EOdd}$ closer to 1, meaning fairness is further improved. Both the original and new approaches provide reasonable performance-fairness trade-offs. 

\textbf{1DCNN-LSTM} \quad The general performance with the new regularisation approach is better than the original approach but worse than massaging, and the new approach achieves the best sensitivity. In terms of fairness, the new approach brings all three metrics closest to 1, and it is the only method that leads to a model satisfying equalised odds. Therefore, the small performance drop compared with massaging is justified by fairness improvements. 

\subsection{MODMA}
We describe the results for MODMA concerning Table \ref{tab:dataset2}. We begin with the performance and bias of models as shown in the ``Base" column.

\begin{table}[]
    \centering
    %\captionsetup{font=scriptsize}
    %\scalebox{0.62}{
    \begin{tabular}{ll|cccccc|c}
         % & & \multicolumn{7}{|c}{\textbf{MODMA}}\\ \cline{3-9}
         & & Base & Aug & Mas & RW & Reg & ROC & Reg+ \\ \hline
         \multirow{18}{*}{\centering \begin{sideways}\textbf{Deep-Asymmetry}\end{sideways}} & \multirow{2}{*}{\centering Accuracy} & 0.9114 & 0.9132 & 0.8740 & 0.8737 & 0.8657 & \textbf{0.9175} & 0.8654 
\\
         & & ±0.0111 & ±0.0116 & ±0.0076 & ±0.0066 & ±0.0122 & ±0.0103 & ±0.0287 \\
         & \multirow{2}{*}{\centering Sensitivity} & 0.8861 & 0.8833 & 0.8306 & 0.8311 & 0.7433 & \textbf{0.9097} & 0.8856 
\\
         & & ±0.0287 & ±0.0236 & ±0.0288 & ±0.0314 & ±0.0259 & ±0.0260 & ±0.0549 \\
         & \multirow{2}{*}{\centering Specificity} & 0.9324 & 0.9379 & 0.9099 & 0.9090 & \textbf{0.9669} & 0.9094 & 0.8487 
\\
         & & ±0.0233 & ±0.0159 & ±0.0104 & ±0.0245 & ±0.0087 & ±0.0280 & ±0.0892 \\
         & \multirow{2}{*}{\centering Precision} & 0.9168 & 0.9222 & 0.8845 & 0.8845 & \textbf{0.9491} & 0.9241 & 0.8399 
\\
         & & ±0.0252 & ±0.0178 & ±0.0086 & ±0.0233 & ±0.0131 & ±0.0249 & ±0.0745 \\
         & \multirow{2}{*}{\centering F1} & 0.9005 & 0.9020 & 0.8562 & 0.8562 & 0.8334 & \textbf{0.9089} & 0.8574
\\
         & & ±0.0129 & ±0.0134 & ±0.0118 & ±0.0094 & ±0.0171 & ±0.0114 & ±0.0210
\\ \cline{2-9}

         & \multirow{2}{*}{\centering $\mathcal{M}_{SP}$} & 1.2564 & 1.2444 & 1.1685 & 1.1466 & 1.0495 & 1.3567 & 1.2111 
         \\
         & & ±0.0979 & ±0.0825 & ±0.1372 & ±0.1280 & ±0.1292 & ±0.0944 & ±0.0833 \\
         & \multirow{2}{*}{\centering $\mathcal{M}_{EOpp}$} & 0.8997 & 0.9228 & 0.8208 & 0.8203 & 0.7503 & \textbf{0.9552} & 0.8944 
\\
         & & ±0.0432 & ±0.0496 & ±0.0518 & ±0.0607 & ±0.0553 & ±0.0448 & ±0.0414 \\
         & \multirow{2}{*}{\centering $\mathcal{M}_{EOdd}$} & 1.8259 & \textbf{1.2236} & 1.7905 & 1.4818 & 1.4715 & 2.3522 & 1.4066 
\\
         & & ±0.5085 & ±0.4127 & ±0.5138 & ±0.5705 & ±0.7018 & ±0.7671 & ±0.1535\\
         & \multirow{2}{*}{\centering $\mathcal{M}_{EAcc}$} & 0.9245 & \textbf{0.9513} & 0.8712 & 0.8783 & 0.8459 & 0.9420 & 0.9235 
\\
         & & ±0.0249 & ±0.0385 & ±0.0202 & ±0.0177 & ±0.0232 & ±0.0282 & ±0.0213 
\\ \hline
         
         \multirow{9}{*}{\centering \begin{sideways}\textbf{GTSAN}\end{sideways}} & Accuracy & \textbf{0.9843} & 0.9811 & 0.9308 & 0.8459 & 0.9308 & 0.9465 & 0.9623 
\\
         & Sensitivity & 0.9672 & 0.9705 & 0.9770 & 0.6984 & \textbf{0.9934} & 0.9672 & 0.9344
\\
         & Specificity & \textbf{1.0000} & 0.9909 & 0.8882 & 0.9819 & 0.8731 & 0.9275 & 0.9879 
\\
         & Precision & \textbf{1.0000} & 0.9900 & 0.8896 & 0.9726 & 0.8783 & 0.9248 & 0.9862
\\
         & F1 & \textbf{0.9833} & 0.9802 & 0.9312 & 0.8130 & 0.9323 & 0.9455 & 0.9596 
\\ \cline{2-9}

         & $\mathcal{M}_{SP}$ & 1.4693 & 1.4335 & 1.4464 & 1.3095 & 1.4542 & 1.7305 & 1.5055 
\\
         & $\mathcal{M}_{EOpp}$ & 1.0625 & 1.0559 & 0.9481 & 0.9574 & \textbf{0.9852} & 1.0625 & 1.1019
\\
         & $\mathcal{M}_{EOdd}$ & $\infty$ & 0.0000 & 4.4536 & 1.2062 & 3.2165 & $\infty$ & \textbf{0.8041}
\\
         & $\mathcal{M}_{EAcc}$ & \textbf{1.0254} & 1.0306 & 0.8952 & 0.9277 & 0.9293 & 0.9193 & 1.0412
\\ \hline

         \multirow{9}{*}{\centering \begin{sideways}\textbf{1DCNN-LSTM}\end{sideways}} & Accuracy & 0.9569 & \textbf{0.9840} & 0.8322 & 0.9808 & 0.9489 & 0.9569 & 0.9808 
\\
         & Sensitivity & 0.9117 & 0.9682 & 0.7915 & \textbf{0.9894} & 0.9152 & 0.9117 & 0.9892 
\\
         & Specificity & 0.9942 & \textbf{0.9971} & 0.8659 & 0.9738 & 0.9767 & 0.9942 & 0.9682 
\\
         & Precision & 0.9923 & \textbf{0.9964} & 0.8296 & 0.9689 & 0.9700 & 0.9923 & 0.9913 
\\
         & F1 & 0.9503 & \textbf{0.9821} & 0.8101 & 0.9790 & 0.9418 & 0.9503 & 0.9786
\\ \cline{2-9}
         & $\mathcal{M}_{SP}$ & 1.5962 & 1.4485 & 1.0005 & 1.3738 & 1.6063 & 1.5962 & 1.4078
\\
         & $\mathcal{M}_{EOpp}$ & 1.1633 & 1.0638 & 0.7298 & \textbf{1.0059} & 1.1543 & 1.1633 & 1.0484 
\\
         & $\mathcal{M}_{EOdd}$ & $\infty$ & $\infty$ & 1.3952 & 2.4783 & 5.9478 & $\infty$  & \textbf{0.9913}
\\
         & $\mathcal{M}_{EAcc}$ & 1.0476 & 1.0203 & 0.8322 & \textbf{0.9915} & 1.0334 & 1.0476 & 1.0189 
\\
    \end{tabular}%}
    \emph{\caption{Summary of performance and fairness results for the \textbf{MODMA} dataset. \emph{Abbreviations and remarks: Same as those in Table \ref{tab:dataset1}.}}
    \label{tab:dataset2}
    }
\end{table}

The performance results from the GTSAN model were consistent with the original work \cite{GTSAN}. We achieved an accuracy of 0.9843 while the authors reported an accuracy of 0.9756 for MODMA. Overall, GTSAN performed best and Deep-Asymmetry performed worst using MODMA. All models had specificity as the best-performing metric and sensitivity as the worst. 

Similar fairness results are obtained for all three models. $\mathcal{M}_{EOpp}$ and $\mathcal{M}_{EAcc}$ stay in the 0.8--1.2 range, but $\mathcal{M}_{EOdd}$ is greater than 1.2, which indicates strong bias in favour of females. GTSAN and 1DCNN-LSTM even have an undefined $\mathcal{M}_{EOdd}$. These results mean that the models only satisfy the more lenient fairness definitions but not the stricter equalised odds framework. To determine which model is the fairest, we observe that GTSAN is fairer than 1DCNN-LSTM across all metrics. Although GTSAN is slightly fairer than Deep-Asymmetry when considering equal opportunity and equal accuracy, Deep-Asymmetry is much fairer than GTSAN in terms of the more stringent equalised odds. Overall, Deep-Asymmetry is therefore the fairest and 1DCNN-LSTM is the most biased. 

We then turn to the bias mitigation results, which are based on the "Base" column and the 5 columns following it. 

\textbf{Deep-Asymmetry} \quad Massaging, reweighing and regularisation cause performance to drop across most metrics while the other two do not. Different methods change $\mathcal{M}_{EOpp}$ and $\mathcal{M}_{EAcc}$ differently. Data augmentation and ROC increase their values while the others decrease their values slightly, but they stay in the range 0.8--1.2 except $\mathcal{M}_{EOpp}$ for regularisation. In terms of $\mathcal{M}_{EOdd}$, all methods except ROC can reduce bias towards females but still fail to bring fairness. Overall, \textbf{data augmentation} produces the best fairness results without sacrificing performance. 

\textbf{GTSAN} \quad Except for data augmentation, all mitigation methods worsen performance, especially for reweighing. The methods generally decrease $\mathcal{M}_{EOpp}$ and $\mathcal{M}_{EAcc}$ slightly. No method results in equalised odds fairness, but reweighing brings $\mathcal{M}_{EOdd}$ down to slightly above 1.2. Although regularisation produces a value of 3.2165 for $\mathcal{M}_{EOdd}$ which is worse than reweighing, performance remains high, especially for sensitivity. Hence, \textbf{regularisation} produces the best performance-fairness trade-off. 

\textbf{1DCNN-LSTM} \quad 
%ROC has no effect on performance. 
Data augmentation and reweighing improve performance across most metrics. Massaging and regularisation worsen performance, especially for massaging. Apart from ROC which does not change fairness, all methods cause $\mathcal{M}_{EOpp}$ and $\mathcal{M}_{EAcc}$ to drop, and massaging even causes $\mathcal{M}_{EOpp}$ to drop below 0.8. No method results in $\mathcal{M}_{EOdd}$ lying between 0.8 and 1.2, but massaging, reweighing and regularisation improve this metric, especially for massaging. Overall, \textbf{reweighing} provides the best performance-fairness trade-off as it improves both performance and fairness. 

Overall, \textbf{in-processing} bias mitigation methods work better for MODMA.

Finally, we compare the results for the proposed method (``Reg+" column) with the original regularisation method (``Reg" column) and the method with the best performance-fairness trade-off.

\textbf{Deep-Asymmetry} \quad Compared with the original approach, the new regularisation approach has comparable accuracy but trades in specificity and precision for sensitivity and F1 score. It improves all fairness metrics by making them closer to 1, but $\mathcal{M}_{EOdd}$ is still above 1.2. Improved regularisation still falls behind data augmentation, the method with the best performance-fairness balance, across most performance and fairness metrics.

\textbf{GTSAN} \quad The new regularisation approach improves performance across all aspects except sensitivity when compared with the original approach. It increases $\mathcal{M}_{EOpp}$ and $\mathcal{M}_{EAcc}$ but does not bring them outside the range 0.8--1.2. It greatly improves equalised odds fairness as it reduces $\mathcal{M}_{EOdd}$ to 0.8041. The model is fair with respect to all three fairness definitions. To conclude, the new regularisation approach achieves a much better performance-fairness trade-off. 

\textbf{1DCNN-LSTM} \quad The new regularisation approach produces performance results comparable with reweighing and even has better precision. Performance is improved across most metrics when compared with the original regularisation approach. Although reweighing leads to slightly better $\mathcal{M}_{EOpp}$ and $\mathcal{M}_{EAcc}$, only the new regularisation approach can result in a fair $\mathcal{M}_{EOdd}$ value. This new approach leads to fairness across all three metrics without sacrificing performance, hence it has the best performance-fairness trade-off. 

\subsection{Rest}
We describe the results for Rest regarding Table \ref{tab:dataset3}. We first mention the performance and bias of models according to the ``Base" column.

\begin{table}[]
    \centering
    %\captionsetup{font=scriptsize}
    %\scalebox{0.62}{
    \begin{tabular}{ll|cccccc|c}
         % & & \multicolumn{7}{|c}{\textbf{Rest}}\\ \cline{3-9}
         & & Base & Aug & Mas & RW & Reg & ROC & Reg+ \\ \hline
         \multirow{18}{*}{\centering \begin{sideways}\textbf{Deep-Asymmetry}\end{sideways}} & \multirow{2}{*}{\centering Accuracy} & 0.9525 & \textbf{0.9531} & 0.9215 & 0.9271 & 0.9299 & 0.9510 & 0.9150
\\
         & & ±0.0047 & ±0.0105 & ±0.0137 & ±0.0137 & ±0.0053 & ±0.0044 & ±0.0184\\
         & \multirow{2}{*}{\centering Sensitivity} & 0.9133 & 0.9030 & 0.8800 & 0.8909 & 0.8548 & \textbf{0.9483} & 0.8939
\\
         & & ±0.0235 & ±0.0385 & ±0.0190 & ±0.0184 & ±0.0124 & ±0.0165 & ±0.0299\\
         & \multirow{2}{*}{\centering Specificity} & 0.9749 & \textbf{0.9816} & 0.9453 & 0.9477 & 0.9728 & 0.9158 & 0.9271
\\
         & & ±0.0100 & ±0.0070 & ±0.0281 & ±0.0283 & ±0.0078 & ±0.0233 & ±0.0386\\
         & \multirow{2}{*}{\centering Precision} & 0.9547 & 0.9662 & 0.9047 & 0.9096 & 0.9476 & \textbf{0.9711} & 0.8798
\\
         & & ±0.0164 & ±0.0121 & ±0.0435 & ±0.0419 & ±0.0142 & ±0.0102 & ±0.0531\\
         & \multirow{2}{*}{\centering F1} & \textbf{0.9332} & 0.9329 & 0.8912 & 0.8992 & 0.8987 & 0.9313 & 0.8851
\\
         & & ±0.0075 & ±0.0171 & ±0.0158 & ±0.0155 & ±0.0077 & ±0.0070 & ±0.0201
\\ \cline{2-9}

         & \multirow{2}{*}{\centering $\mathcal{M}_{SP}$} & 0.5394 & 0.5350 & 0.5895 & 0.5862 & 0.5583 & 0.5606 & 0.6039
         \\
         & & ±0.0251 & ±0.0141 & ±0.0607 & ±0.0525 & ±0.0200 & ±0.0229 & ±0.0555 \\
         & \multirow{2}{*}{\centering $\mathcal{M}_{EOpp}$} & 1.0254 & 1.0338 & \textbf{1.0213} & 1.0273 & 1.0292 & 1.0373 & 1.0372
\\
         & & ±0.0107 & ±0.0091 & ±0.0223 & ±0.0181 & ±0.0185 & ±0.0134 & ±0.0204 \\
         & \multirow{2}{*}{\centering $\mathcal{M}_{EOdd}$} & 1.3152 & \textbf{0.9919} & 1.3274 & 1.2849 & 1.4427 & 1.7713 & 1.1601
\\
         & & ±0.5703 & ±0.4860 & ±0.4359 & ±0.5493 & ±0.7563 & ±0.7721 & ±0.2408 \\
         & \multirow{2}{*}{\centering $\mathcal{M}_{EAcc}$} & 1.0211 & 1.0275 & \textbf{1.0108} & 1.0116 & 1.0291 & 1.0167 & 1.0128
\\
         & & ±0.0050 & ±0.0114 & ±0.0228 & ±0.0290 & ±0.0139 & ±0.0079 & ±0.0218
\\ \hline

         \multirow{9}{*}{\centering \begin{sideways}\textbf{1DCNN-LSTM}\end{sideways}} & Accuracy & 0.8894 & 0.8711 & 0.8263 & \textbf{0.8908} & 0.8859 & 0.8824 & 0.8690
\\
         & Sensitivity & 0.8011 & 0.8361 & 0.7735 & 0.8416 & \textbf{0.8582} & 0.8048 & 0.8287
\\
         & Specificity & \textbf{0.9435} & 0.8927 & 0.8588 & 0.9209 & 0.9028 & 0.9299 & 0.8938
\\
         & Precision & \textbf{0.8969} & 0.8270 & 0.7706 & 0.8672 & 0.8442 & 0.8758 & 0.8272
\\
         & F1 & 0.8463 & 0.8315 & 0.7721 & \textbf{0.8542} & 0.8511 & 0.8388 & 0.8280
\\ \cline{2-9}
         & $\mathcal{M}_{SP}$ & 0.5931 & 0.6049 & 0.9514 & 0.6582 & 0.6116 & 0.6580 & 0.6356
\\
         & $\mathcal{M}_{EOpp}$ & 0.9778 & 1.0474 & 1.1480 & 1.1143 & 1.0121 & \textbf{0.9973} & 1.0218
\\
         & $\mathcal{M}_{EOdd}$ & 1.4678 & 0.7357 & 2.9656 & 1.0892 & 0.9570 & 2.0969 & \textbf{1.0149}
\\
         & $\mathcal{M}_{EAcc}$ & 1.0153 & 1.0535 & 0.9485 & 1.0469 & 1.0183 & \textbf{0.9942} & 1.0223
\\
    \end{tabular}%}
    \emph{\caption{Summary of performance and fairness results for the \textbf{Rest} dataset. \emph{Abbreviations and remarks: Identical to those in Table \ref{tab:dataset1}.}}
    \label{tab:dataset3}
    }
\end{table}

Overall, Deep-Asymmetry has better performance than 1DCNN-LSTM. For both models, specificity is the greatest and sensitivity is the lowest among all performance metrics.

Moving on to fairness, for both models, $\mathcal{M}_{EOpp}$ and $\mathcal{M}_{EAcc}$ are close to 1 but $\mathcal{M}_{EOdd}$ is greater than 1.2, which signifies bias towards males. This means both models only satisfy equal opportunity and equal accuracy. The value of $\mathcal{M}_{EOdd}$ for 1DCNN-LSTM is 1.4678, which is greater than that for Deep-Asymmetry, 1.3152. Hence, 1DCNN-LSTM is more biased than Deep-Asymmetry when trained with Rest.

We then describe whether bias mitigation methods are effective by comparing the values in the ``Base" column and the 5 columns following it.

\textbf{Deep-Asymmetry} \quad Massaging, reweighing and regularisation result in a small performance drop across all metrics but the other two methods do not. All methods have little effect on $\mathcal{M}_{EOpp}$ and $\mathcal{M}_{EAcc}$. In terms of $\mathcal{M}_{EOdd}$, ROC produces the worst fairness. Although reweighing reduces $\mathcal{M}_{EOdd}$, only data augmentation can bring its value below 1.2 and very close to 1. Overall, \textbf{data augmentation} succeeds in producing a fair model without losing performance. 

\textbf{1DCNN-LSTM} \quad Both pre-processing methods cause performance to decrease across most metrics. Both in-processing methods have varied effects on different performance metrics. They increase sensitivity but decrease specificity and precision, while accuracy and F1 score have minimal changes. ROC has little effect on performance. All methods increase $\mathcal{M}_{EOpp}$ but some increase and others decrease $\mathcal{M}_{EAcc}$. Still, these two values remain in the 0.8--1.2 range. Regarding $\mathcal{M}_{EOdd}$, both in-processing methods bring their values close to 1, especially for regularisation. Data augmentation causes the model to be biased towards the other group, the females, instead. The other two methods increase bias towards males. Overall, reweighing and regularisation produce models that are fair across all three metrics without sacrificing performance, but \textbf{regularisation} brings metrics even closer to 1. 

Overall, \textbf{pre- and in-processing} methods are more effective at mitigating bias for Rest.

We end this subsection with the results for the new regularisation approach concerning the ``Reg+" column. 

\textbf{Deep-Asymmetry} \quad The new approach has better sensitivity and specificity but worse accuracy, specificity and F1 score than the original approach. $\mathcal{M}_{EOpp}$ and $\mathcal{M}_{EAcc}$ do not change much, but the new regularisation approach brings $\mathcal{M}_{EOdd}$ down to 1.1601. This means the model now satisfies equalised odds fairness. Overall, data augmentation still has better performance and fairness results, but the new regularisation approach is slightly fairer in terms of equal accuracy. 

\textbf{1DCNN-LSTM} \quad Compared with the original regularisation approach, the new approach results in a small decline in performance across all metrics. In terms of fairness, the original approach is slightly fairer in terms of equal opportunity and equal accuracy while the new approach is fairer in terms of equalised odds. Both approaches are acceptable, and the choice depends on how important equalised odds is. 

\section{Analysis and Discussion}
This section is divided into two. In the first part, we use the above experimental results to respond to the RQs. In the second part, we explain some other findings and discuss their potential causes and/or implications. 

\subsection{RQs}
\subsubsection{RQ1. Is there bias in existing EEG-based depression datasets and algorithms?}

All three datasets have bias. With reference to Table \ref{tab:datasets}, all three datasets are imbalanced across genders but not heavily imbalanced. The most imbalanced dataset is Mumtaz, with around 76\% more males than females. %Therefore, the minority class is female. 
Females are also considered the minority for MODMA, in which the number of males and females has a relative difference of 65\%. The least imbalanced dataset is Rest. For Rest, the number of females is around 57\% greater than males, so males are the minority. 

% Overall, the model is fair with respect to equal opportunity and equal accuracy, the relaxed notions of separation, across all datasets, but its fairness is varied when considering equalised odds. 
% Overall, the model satisfies equal opportunity and equal accuracy across datasets, but not the stricter equalised odds. 
% Overall, 1DCNN-LSTM is fair based on equal opportunity and equal accuracy across datasets but is unfair according to equalised odds. 

All three algorithms are acceptably fair with respect to equal opportunity and equal accuracy but not equalised odds. The only model that satisfies equalised odds is Deep-Asymmetry trained with the Mumtaz dataset. Models can be biased towards different groups when trained with different datasets. Different models trained with the same dataset, such as Mumtaz, can be biased towards different groups but they can also be biased towards the same group, e.g.\ all models trained with MODMA are biased towards females and those trained with Rest are biased towards males. 

\subsubsection{RQ2. What is the performance-fairness trade-off of existing bias mitigation strategies? }

We observe similar trends across different datasets. 

While data augmentation and ROC both have little effect on performance, they have different effectiveness in mitigating bias. ROC is not very effective and can sometimes exacerbate bias. Although data augmentation only leads to small changes in fairness metrics, it can sometimes give the fairest results.

Massaging and regularisation usually result in the greatest drop in performance but also the greatest improvement in fairness. Regularisation often has a less adverse effect on performance and better fairness improvements than massaging, so regularisation has a better performance-fairness trade-off. It even has the best trade-off in many cases, as evidenced in the last section.

Reweighing lies between the above two groups. It usually leads to a small performance drop and small fairness improvements. Nevertheless, it sometimes brings biased models to acceptable fairness. 


% In-processing methods, especially \textbf{regularisation}, are effective at mitigating bias and they usually provide good performance-fairness trade-offs. ROC is the least effective bias mitigation method. 

\subsubsection{RQ3. Can we make existing EEG-based depression detection algorithms fairer while accurate? }

It is sometimes possible to make depression detection fairer without damaging performance as in data augmentation for the Deep-Asymmetry algorithm with MODMA and Rest and the proposed method for 1DCNN-LSTM with MODMA. Nevertheless, fairness improvements usually come with a performance drop. Therefore, the usual intended goal is turning strongly biased algorithms into acceptably fair ones without largely compromising performance. The original regularisation approach can usually accomplish this with the best performance-fairness trade-offs among existing methods but the new approach is better. The new method has comparable or even better performance and fairness results at the same time in most cases. Even if the performance is slightly behind that of the original approach, this is justified by an improvement in fairness. We conclude that it is possible to make existing EEG-based depression detection algorithms fairer while at an acceptably high performance. 

\subsection{Discussion}
\label{sec:discussion}

As mentioned in Section \ref{sec:implm_training}, the GTSAN method had little sign of learning when trained with Rest. The performance was also fair when trained with Mumtaz. We found overfitting and underfitting problems with this model. When the weights are tightly restricted or the dropout rate is high, the model underfits. However, the model easily overfits without strong regularisation. These results mean that the model is not generalisable to other datasets and is susceptible to memorisation. One potential reason for the undesirable performance is the manually extracted features might not be strong enough for general depression detection, but only capture characteristics specific to a particular dataset. 

We now move the topic of discussion to fairness. The fairness results illustrate the importance of choosing a suitable fairness definition and corresponding metric, which is stressed in the literature \cite{eq_opp}. Regardless of the bias mitigation performed, models trained using datasets with females as the minority generally have $\mathcal{M}_{SP}$ greater than 1 and models trained using datasets with males as the minority have $\mathcal{M}_{SP}$ less than 1. This means the models classify a higher proportion of females than males as depressed, which is expected for reasonable datasets as the depression base rate of females is greater. These observations verify that statistical parity is not suitable for evaluating fairness for our task. Besides, the results confirm that it is more difficult for models to satisfy the stricter equalised odds framework. All models satisfy equal opportunity and equal accuracy without needing bias mitigation. It would be meaningless if we just consider these two relaxed notions of fairness. 

We observe that data augmentation and reweighing generally cause fairness metrics, especially $\mathcal{M}_{EOdd}$, to decrease, while ROC generally causes the metrics to increase. Massaging and regularisation are less consistent in this regard. They usually result in a decrease in metrics but sometimes lead to an increase. This suggests that data augmentation, reweighing and ROC are less specific methods than the other two. The reason is that regardless of the nature of datasets and models, data augmentation and reweighing usually reduce bias towards the minority group, while ROC reduces bias in favour of the majority. These methods can still be useful when it is clear whether we want to increase or decrease the metrics after evaluating model fairness. However, massaging and regularisation might have the advantage of being adaptive to the dataset and model used for bias mitigation. 

The above discussion also provides insights into bias mitigation using multiple methods simultaneously. Based on the original value of the metrics, a suitable combination of methods that increase and decrease metrics can lead to better fairness. For example, combining data augmentation with ROC produces $\mathcal{M}_{EOdd} = 0.9249 \pm 0.5089$ for the Deep-Asymmetry model trained using Mumtaz, which is closer to 1 than that without any bias mitigation, with data augmentation only and with ROC only. For the 1DCNN-LSTM model trained using Rest, we also obtain a similar observation, with $\mathcal{M}_{EOdd}$ = 0.9544 when both data augmentation and ROC are carried out. 

Finally, we observe that there is no single bias mitigation method that achieves better performance and fairness than the others in \textbf{all} cases, which is in line with existing work \cite{concl}. The results depend on specifics such as the fairness metric and dataset. Nevertheless, there are methods that \textbf{generally} have better performance-fairness balance, such as data augmentation and regularisation. The best bias mitigation approach would depend on the task itself and preference on performance or fairness.

\chapter{Summary and Conclusions}
\label{chap:concl}
\emph{In this chapter, we conclude the dissertation with some pointers to future work with respect to the limitations of this study and a summary.
%of the study.
}

\section{Limitations}
One limitation of this study is that we only work on group fairness with respect to gender but there are other sensitive attributes such as age and race. It is important to conduct fairness evaluation concerning these attributes as well because there are groups that were historically discriminated against in other tasks. However, this depends on the availability of public datasets that have this sensitive information and contain data from a sufficient number of individuals in each group defined by the sensitive attribute. 

Besides, for direct comparability of results, we extracted parts of the datasets that were collected under similar conditions and ignored the rest. Nevertheless, the remaining data such as eyes-closed EEG data are also valuable and can be used for depression detection. With the difference in performance already known, one future direction would be to investigate fairness for eyes-closed EEG data and compare the fairness evaluation and bias mitigation results between eyes-closed and eyes-open data. 

\section{Summary}
In this study, we evaluated the gender fairness of three existing algorithms for depression detection using EEG data trained across three different datasets. We then applied different pre-, in- and post-processing bias mitigation techniques. We also proposed a bias mitigation approach that improved upon the original regularisation method. The new approach modified the regularisation terms and training process. The newly introduced hyperparameters can allow more flexible control of the balance between performance and fairness. This is the first time such an investigation on ML fairness and bias mitigation has been conducted for EEG-based depression detection.

Our findings can be summarised as follows. Existing datasets and algorithms can be biased in favour of different genders. For each dataset, the models trained satisfy the weaker equal opportunity and equal accuracy frameworks but usually not equalised odds. Pre- and in-processing techniques are more effective at mitigating bias, but different techniques have different performance-fairness trade-offs. The in-processing technique regularisation is especially promising as it has the best trade-offs in many settings. The proposed method can produce comparable or even better performance-fairness trade-offs than the original regularisation approach.

To conclude, we showed that the bias of ML algorithms for EEG-based depression detection can usually be effectively mitigated at a low or no cost of performance.
